Scalar Representation of 2D Steady Vector Fields

We introduce a representation of a 2D steady vector field ${{\mathbf v}}$ by two scalar fields $a$, $b$, such that the isolines of $a$ correspond to stream lines of ${{\mathbf v}}$, and $b$ increases with constant speed under integration of ${{\mathbf v}}$. This way, we get a direct encoding of stream lines, i.e., a numerical integration of ${{\mathbf v}}$ can be replaced by a local isoline extraction of $a$. To guarantee a solution in every case, gradient-preserving cuts are introduced such that the scalar fields are allowed to be discontinuous in the values but continuous in the gradient. Along with a piecewise linear discretization and a proper placement of the cuts, the fields $a$ and $b$ can be computed. We show several evaluations on non-trivial vector fields.

==> figures/dummy.tex <==
%!TEX root = ../FlowMapModification.tex
%
\begin{tikzpicture}
    \input{colormaps}

    \tikzstyle{image} = [inner sep=0.5, outer sep=0.5, node distance = 0.5cm and 0.5cm]

    \node[image, align=right] (image1) {
        \includegraphics[height=7.0cm]{figures/dummy0}%
    };

    \node[image, anchor=north west, shift={(0.25cm, 0mm)}] (image2) at (image1.north east)
    {
        \includegraphics[height=3.2cm]{figures/dummy1}%
    };

    \node[image, anchor=south west, shift={(0.25cm, 0mm)}] (image3) at (image1.south east)
    {
        \includegraphics[height=3.2cm]{figures/dummy2}%
    };

    \node[anchor=south east, xshift=-0.5cm] at (image1.south west){
        \begin{axis}[
        scale only axis,
        height=6.0cm,
        width=0.6cm,
        hide axis,
        xmin=0, xmax=1,
        ymin=0, ymax=10,
        colorbar,
        colorbar/width=0.3cm,
        %colormap name={red-yellow-blue},
        colormap name={viridis},
        point meta min=0,
        point meta max=10,
        colorbar style={
          title=$t$,
          title style={yshift=-1ex,},
          scaled ticks=false,
          yticklabel pos=left,
          ytick = {0,  10},
          yticklabels = {0, 10}
        }
        ]
        \end{axis}
    };

    \node[anchor=south west, xshift=-0.0cm] at (image3.south east){
        \begin{axis}[
        scale only axis,
        height=6.0cm,
        width=0.6cm,
        hide axis,
        xmin=0, xmax=1,
        ymin=0, ymax=10,
        colorbar,
        colorbar/width=0.3cm,
        %colormap name={brown-white-teal},
        colormap name={magma},
        point meta min=0,
        point meta max=10,
        colorbar style={
          title=$\tau$,
          title style={yshift=-1ex,},
          scaled ticks=false,
          yticklabel pos=right,
          ytick = {0,  10},
          yticklabels = {0, 10}
        }]
        \end{axis}
    };
\end{tikzpicture}%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../FlowMapModification"
%%% End:

